Phase-Field Methods for Spectral Shape and Topology Optimization

We optimize a selection of eigenvalues of the Laplace operator with Dirichlet or Neumann boundary conditions by adjusting the shape of the domain on which the eigenvalue problem is considered. Here, a phase-field function is used to represent the shapes over which we minimize. The idea behind this method is to modify the Laplace operator by introducing phase-field dependent coefficients in order to extend the eigenvalue problem on a fixed design domain containing all admissible shapes. The resulting shape and topology optimization problem can then be formulated as an optimal control problem with PDE constraints in which the phase-field function acts as the control. For this optimal control problem, we establish first-order necessary optimality conditions and we rigorously derive its sharp interface limit. Eventually, we present and discuss several numerical simulations for our optimization problem.

==> Neumann2D_err_lam1_eps_over_c.tikz.tex <==

\begin{tikzpicture}

\begin{axis}[%
width=0.5\textwidth,
height=5cm,
%scale only axis,
xmin=0.05,
xmax=0.2,
xminorticks=true,
xlabel={$c$},
%ymode=log,
ymin=0.000000,
ymax=0.025,
yminorticks=true,
%ylabel={$\eta_{\eps,1}^h$},
axis background/.style={fill=white},
cycle list name=black white,
%
%title={$minimize lam1$},
legend style={legend cell align=left, align=left, draw=white!15!black},
legend pos={north west}
]
\addplot 
  table[row sep=crcr]{%
0.2	0.0210711452058911\\
0.15	0.0101998112684917\\
0.1	0.000860747132642542\\
0.05	0.00766541002154925\\
};
\addlegendentry{ $\eps =0.04$}

\addplot+ 
  table[row sep=crcr]{%
0.2	0.00906763348528877\\
0.15	0.00346270674785562\\
0.1	0.00132846794146505\\
0.05	0.00549607748320424\\
};
\addlegendentry{ $\eps = 0.02$}

\addplot+ 
  table[row sep=crcr]{%
0.2	0.00423490969525964\\
0.15	0.00136414852512427\\
0.1	0.00102724869836283\\
0.05	0.00306566635837388\\
};
\addlegendentry{ $\eps = 0.01$ }

\addplot+ 
  table[row sep=crcr]{%
0.2	0.00210003708902769\\
0.15	0.000640443002615109\\
0.1	0.000556358890333743\\
0.05	0.00156395979361604\\
};
\addlegendentry{ $\eps = 0.005$}

\end{axis}

\end{tikzpicture}%
